A Validity Perspective on Evaluating the Justified Use of Data-driven Decision-making Algorithms

Recent research increasingly brings to question the appropriateness of using predictive tools in complex, real-world tasks. While a growing body of work has explored ways to improve value alignment in these tools, comparatively less work has centered concerns around the fundamental justifiability of using these tools. This work seeks to center validity considerations in deliberations around whether and how to build data-driven algorithms in high-stakes domains. Toward this end, we translate key concepts from validity theory to predictive algorithms. We apply the lens of validity to re-examine common challenges in problem formulation and data issues that jeopardize the justifiability of using predictive algorithms and connect these challenges to the social science discourse around validity. Our interdisciplinary exposition clarifies how these concepts apply to algorithmic decision making contexts. We demonstrate how these validity considerations could distill into a series of high-level questions intended to promote and document reflections on the legitimacy of the predictive task and the suitability of the data.

==> perspective/plans_for_future.tex <==
\subsection{Future directions}
We intend to conduct a series of studies described below to develop, validate, and evaluate our protocol. 

First, we will formulate sub-questions for each top-level question block described in the previous section. We will solicit feedback on these draft questions through workshops with the relevant researchers, community partners, and algorithm developers who have prior experience defining, designing, developing and deploying data-driven decision-making algorithms. We will present our protocol at these workshops and collaborate with workshop participants to generate a set of best practices and to refine and expand our protocol. %Insights from these workshop will be made available as a public website. Once the website is launched, we will seek and integrate additional input from other researchers and community partners.

Second, based on these workshops, we will create and publish a set of resources and artifacts as components of a framework to support replication. These may include: a suite of tools (e.g., explanation tools) that can facilitate the deliberation, a database repository of questionnaires and deliberation protocols researchers use in the studies, an interactive tool for suggesting validity metrics based on study characteristics, a taxonomy of design and deployment features to support AI system design in the field, and a set of designer insight cards to support reflection on common challenges for community stakeholders to evaluate and justify the use of the decision-making algorithm.

Third, as academic instructors we will integrate the protocol into our educational programs. Students in courses with capstone projects can apply the protocol in their projects, providing us with the opportunity to
%structuring their evaluation as a conceptual replication. 
observe how students use the protocol to investigate and deliberate validity issues as they navigate the project design. Observing how (relative) novices apply the protocol to diverse projects affords the opportunity to identify gaps, shortcomings, and confusion with the protocol. This will guide us in validating portions of the framework that work and refining portions that do not.

Throughout this process we will ground our approach in the validity perspective offered here. More broadly, we hope that %our interdisciplinary presentation of a framework for evaluating validity in predictive algorithms 
this framework will energize lines of work on validity and the related issues of reliability in data-driven decision-making algorithms. 

